Fast Search-By-Classification for Large-Scale Databases Using Index-Aware Decision Trees and Random Forests

The vast amounts of data collected in various domains pose great challenges to modern data exploration and analysis. To find "interesting" objects in large databases, users typically define a query using positive and negative example objects and train a classification model to identify the objects of interest in the entire data catalog. However, this approach requires a scan of all the data to apply the classification model to each instance in the data catalog, making this method prohibitively expensive to be employed in large-scale databases serving many users and queries interactively. In this work, we propose a novel framework for such search-by-classification scenarios that allows users to interactively search for target objects by specifying queries through a small set of positive and negative examples. Unlike previous approaches, our framework can rapidly answer such queries at low cost without scanning the entire database. Our framework is based on an index-aware construction scheme for decision trees and random forests that transforms the inference phase of these classification models into a set of range queries, which in turn can be efficiently executed by leveraging multidimensional indexing structures. Our experiments show that queries over large data catalogs with hundreds of millions of objects can be processed in a few seconds using a single server, compared to hours needed by classical scanning-based approaches.

==> figures/intro/mainfigure.tex <==
% Requires \usepackage{fontawesome5}
% Requires \usetikzlibrary{shapes, shapes.geometric, shapes.arrows, arrows, patterns, positioning, calc}
\tikzstyle{positive}=[
    rectangle, 
    draw = none,
    color=red,
	minimum size = 1.2em,
]
%
\tikzstyle{negative}=[
    rectangle, 
    color=blue,
	minimum size = 1.2em,
]
%
\tikzstyle{module}=[
    rectangle, 
    draw = teal!50, 
	fill = teal!50,
	minimum height = 1.5em,
]
%
\tikzstyle{database}=[
    rectangle, 
    color=teal!80,
    minimum width  = 1.2em,
    minimum height = 1.2em,
    font=\Huge,
]
%
\tikzstyle{index}=[
    isosceles triangle,
    isosceles triangle apex angle = 60,
    rotate=90,
    fill = teal!80,
    minimum size = 1.5em,
    anchor=apex,
]
%
\tikzstyle{arrow} = [thick,->,>=stealth, shorten >=1pt]
%
\tikzstyle{customlabel} = [color=black]
\newcommand{\trainnum}{3} 
\newcommand{\testnum}{14} 
%
\begin{tikzpicture}[scale=0.5]
    % Queries
    \draw[black, dashed, fill=black!5] (-0.8, 0.8) rectangle (3.8, -3.8);
    \foreach \i in {0,...,\trainnum}{
        \foreach \j in {0,...,\trainnum}{
            \ifthenelse{\i<1}{
                \node[positive] (pos\i\j) at (\j,-\i) {\faIcon[regular]{file-image}};
            }{
                \node[negative] (neg\i\j) at (\j,-\i) {\faIcon[regular]{file-image}};    
            }
        }
    }
    \foreach \i in {0,...,3}{
        \foreach \j in {5,...,7}{
            \ifthenelse{\i>2}{
                \node[positive] at (\j,-\i) {\faIcon[regular]{file-image}};
            }{
                \node[negative] at (\j,-\i) {\faIcon[regular]{file-image}};    
            }
        }
    }
    \draw[black, dashed, fill=black!5, opacity=.5] (4.2, 0.8) rectangle (7.8, -3.8);
    %
    \foreach \i in {0,...,3}{
        \foreach \j in {9,...,11}{
            \ifthenelse{\i=2}{
                \node[positive] at (\j,-\i) {\faIcon[regular]{file-image}};
            }{
                \node[negative] at (\j,-\i) {\faIcon[regular]{file-image}};    
            }
        }
    }
    \draw[black, dashed, fill=black!5, opacity=.5] (8.2, 0.8) rectangle (11.8, -3.8);
    % System
    \draw[teal, dashed, fill=teal!5] (-0.8, -4.5) rectangle (11.8, -9.8);
    \node[module] (featurizer) at (1.0, -5.5) {Featurizer};
    \node[module, right=1.5em of featurizer] (ml) {ML Algorithm};
    \node[module, right=1.5em of ml] (cls) {Classifier};
    \node[database, below=1em of ml] (db) {\faIcon{database}};
    \node[index, below left=1.2em and -1em of db] (idx1) {};
    \node[index, below left=1.2em and 2em of db] (idx2) {};
    \node[index, below left=1.2em and -4em of db] (idx3) {};
    % Background
    \draw[black, dashed, fill=black!5] (-0.8, -10.2) rectangle (11.8, -14.8);
    \foreach \i in {11,...,14}{
        \foreach \j in {0,...,11}{
            \ifthenelse{\i=11}{
                \node[positive] (res\i\j) at (\j,-\i) {\faIcon[regular]{file-image}};
            }{
                \node[negative] (res\i\j) at (\j,-\i) {\faIcon[regular]{file-image}};    
            }
        }
    }
    \draw[arrow] (featurizer.east)--(ml.west);
    \draw[arrow] (ml.east)--(cls.west);
    \draw[arrow] (cls.south)--(db.north);
    \draw[arrow] (idx1.apex)--(db.south);
    \draw[arrow] (idx2.apex)--(db.south);
    \draw[arrow] (idx3.apex)--(db.south);
\end{tikzpicture}


==> figures/intro/motivation.tex <==
\begin{tikzpicture}
\begin{groupplot}[
    group style={
    group name=boxes,
    group size=2 by 1,
    xlabels at=all,
    ylabels at=all,
    horizontal sep=1cm,
    },
    width=4.5cm,
    height=4.5cm,
    xmin=0, xmax=8,
    ymin=0, ymax=8,
    xtick distance = 1,
    ytick distance = 1,
    xlabel={Feature 1},
    ylabel={Feature 2},
    colormap={allblack}{rgb255(0cm)=(0,0,0) rgb255(5cm)=(0,0,0)},
    scatter/classes={
        a={mark=*, fill=teal, draw=black},%
        b={mark=square*, fill=red, draw=black}
    },
]
\nextgroupplot[title={Decision Tree}]
 \addplot[
        scatter, 
        only marks,
        scatter src=explicit symbolic, 
        mark size=1.4
    ]
    table [x=x, y=y, meta=label]{%
    x  y  label
    3.33394530526422 4.28332468205821 a
    3.17961674705532 3.8276831961824 a
    3.1134149122849 3.61307999982826 a
    5.60910242314673 2.99546048394039 b
    2.97163988750002 3.47723841871636 a
    2.99925801790606 1.53957024838567 a
    2.36283551754169 5.00502647488495 b
    2.99504704134307 5.94584345780937 a
    2.81467117021089 2.79180828538485 a
    2.82965013702828 5.16780439921386 a
    3.38976636653516 2.76941793800773 a
    2.97066892412022 4.58766176040534 a
    3.65367051483291 2.7019912395526 a
    1.62736505997928 3.61338753840246 a
    2.98426576777732 5.33370121321312 a
    2.88585260484527 5.87698901499805 a
    2.84139140515367 3.71710347782753 a
    3.36416590922588 5.00698637275478 b
    3.34743162321116 3.47217929011223 a
    3.2962052490147 4.10497541198083 a
    4.41281456182071 4.53299453165984 b
    1.28819289620032 3.75446194851244 a
    3.10205695804627 5.52159086981174 a
    4.17299060616253 3.57889463322735 b
    2.91013734072135 4.32434508106371 a
    4.25615589424161 3.24005281647642 a
    5.13567148165735 5.45525060039834 b
    3.39670808040643 3.29458420261846 a
    5.23828180412047 3.11386743344958 b
    0.901736605849352 2.8426793108164 a
    4.66438952924408 3.42040198870465 b
    5.05252962162291 3.30652980844534 a
    3.66206683708891 2.85621873615841 a
    2.95846583766988 3.43468639885209 a
    4.58152067710274 4.49390607557343 b
    3.16295533454344 2.07215485437621 a
    2.64290994059636 4.58668118769647 a
    5.59989124731089 2.43869947510318 b
    3.11964154124991 2.69753113721211 a
    2.91427913928509 5.78273397261983 a
    2.24983147265599 0.512453776052884 a
    3.79210543323041 5.24057624249581 b
    5.17458363813847 1.57840449979178 b
    3.65263068962923 3.83194879032914 a
    3.89188184233168 6.0156473385641 b
    1.87755651429736 2.47926625295766 a
    3.20563412433338 4.8299503177551 a
    3.65847289964058 4.35594649785007 b
    4.7504116645498 3.69168819694295 b
    3.03061711322473 4.31718036376117 a
    3.10489468313105 5.33195055037207 a
    3.26816013529554 4.62166949592003 a
    2.85256923790864 4.60921659325744 a
    2.83054876199145 3.00466942808038 a
    3.19985785504756 5.68037474278882 a
    4.67106819732058 2.86732604384515 a
    4.11654344712219 3.82843974380613 b
    3.94097247568952 1.71923606187619 a
    3.50267815522516 2.89885565070775 a
    4.94421447203834 5.92899023433706 b
    4.85508387727516 2.47815787564363 b
    3.19665605019201 5.69445112855963 a
    2.82604033137985 4.05621567046909 a
    3.435642639206 2.23484625537744 a
    3.20447379105593 4.25117341307022 a
    2.97154660000271 6.68381239979278 a
    2.89625824026687 3.61021175006633 a
    2.76930180497786 2.85194062003077 a
    3.48470699044717 3.03599187091698 a
    3.2615625757792 4.40918752625346 a
    3.31908931625676 5.95082391506104 a
    3.40772777457981 1.35402447498146 a
    5.63590334857413 3.23046304809946 b
    3.46418780499208 5.2532962753061 a
    4.81804015863207 3.24356183900056 a
    3.32574801852368 5.34997548719981 a
    2.98254664216517 5.16661394243277 a
    4.57311496229195 4.45931319631445 b
    2.95144223357696 4.76582546007239 a
    2.64874055869206 3.33711558353641 a
    2.86394877458514 4.69859130351621 a
    3.05000367541074 5.73240861105973 a
    3.82181285583226 3.74547112789699 b
    4.4239026177482 2.12757243927978 b
    2.73327988891727 3.04713402219221 a
    3.66697628789954 2.6651037751997 a
    2.68636437091379 3.74003269642794 a
    3.11055071205753 4.27343615977398 a
    3.23061499554796 3.23930038112248 a
    3.03895675529012 3.43560203374447 a
    3.63877987049824 0.402564002310837 a
    2.04678419358542 4.52234144069177 a
    };
    % Begin Decision Tree
    \addplot[surf,mesh/rows=2,patch type=rectangle, fill=teal, fill opacity=0.1, draw=white]
    coordinates {
    (0,0) (0,8)
    (8,0) (8,8)
    };
    \addplot[draw=none, surf, mesh/rows=2, patch type=rectangle, fill=red, fill opacity=0.3]
    coordinates {
    (0,4.9) (3.65,4.9)
    (0,5.1) (3.65,5.1)
    };
    \addplot[surf,mesh/rows=2,patch type=rectangle, fill=red, fill opacity=0.3]
    coordinates {
    (4.3,0.0) (4.58,0.0)
    (4.3,3.2) (4.58,3.2)
    };
    \addplot[surf,mesh/rows=2,patch type=rectangle, fill=red, fill opacity=0.3]
    coordinates {
    (3.65,3.35) (8.0,3.35)
    (3.65,8.0) (8.0,8.0)
    };
    \addplot[surf,mesh/rows=2,patch type=rectangle, fill=red, fill opacity=0.3]
    coordinates {
    (4.8,0.0) (8.0,0.0)
    (4.8,3.2) (8.0,3.2)
    };
    \nextgroupplot[title={Decision Branches}]
    \addplot[
        scatter, 
        only marks,
        scatter src=explicit symbolic, 
        mark size=1.4
    ]
    table [x=x, y=y, meta=label]{%
    x  y  label
   3.33394530526422 4.28332468205821 a
    3.17961674705532 3.8276831961824 a
    3.1134149122849 3.61307999982826 a
    5.60910242314673 2.99546048394039 b
    2.97163988750002 3.47723841871636 a
    2.99925801790606 1.53957024838567 a
    2.36283551754169 5.00502647488495 b
    2.99504704134307 5.94584345780937 a
    2.81467117021089 2.79180828538485 a
    2.82965013702828 5.16780439921386 a
    3.38976636653516 2.76941793800773 a
    2.97066892412022 4.58766176040534 a
    3.65367051483291 2.7019912395526 a
    1.62736505997928 3.61338753840246 a
    2.98426576777732 5.33370121321312 a
    2.88585260484527 5.87698901499805 a
    2.84139140515367 3.71710347782753 a
    3.36416590922588 5.00698637275478 b
    3.34743162321116 3.47217929011223 a
    3.2962052490147 4.10497541198083 a
    4.41281456182071 4.53299453165984 b
    1.28819289620032 3.75446194851244 a
    3.10205695804627 5.52159086981174 a
    4.17299060616253 3.57889463322735 b
    2.91013734072135 4.32434508106371 a
    4.25615589424161 3.24005281647642 a
    5.13567148165735 5.45525060039834 b
    3.39670808040643 3.29458420261846 a
    5.23828180412047 3.11386743344958 b
    0.901736605849352 2.8426793108164 a
    4.66438952924408 3.42040198870465 b
    5.05252962162291 3.30652980844534 a
    3.66206683708891 2.85621873615841 a
    2.95846583766988 3.43468639885209 a
    4.58152067710274 4.49390607557343 b
    3.16295533454344 2.07215485437621 a
    2.64290994059636 4.58668118769647 a
    5.59989124731089 2.43869947510318 b
    3.11964154124991 2.69753113721211 a
    2.91427913928509 5.78273397261983 a
    2.24983147265599 0.512453776052884 a
    3.79210543323041 5.24057624249581 b
    5.17458363813847 1.57840449979178 b
    3.65263068962923 3.83194879032914 a
    3.89188184233168 6.0156473385641 b
    1.87755651429736 2.47926625295766 a
    3.20563412433338 4.8299503177551 a
    3.65847289964058 4.35594649785007 b
    4.7504116645498 3.69168819694295 b
    3.03061711322473 4.31718036376117 a
    3.10489468313105 5.33195055037207 a
    3.26816013529554 4.62166949592003 a
    2.85256923790864 4.60921659325744 a
    2.83054876199145 3.00466942808038 a
    3.19985785504756 5.68037474278882 a
    4.67106819732058 2.86732604384515 a
    4.11654344712219 3.82843974380613 b
    3.94097247568952 1.71923606187619 a
    3.50267815522516 2.89885565070775 a
    4.94421447203834 5.92899023433706 b
    4.85508387727516 2.47815787564363 b
    3.19665605019201 5.69445112855963 a
    2.82604033137985 4.05621567046909 a
    3.435642639206 2.23484625537744 a
    3.20447379105593 4.25117341307022 a
    2.97154660000271 6.68381239979278 a
    2.89625824026687 3.61021175006633 a
    2.76930180497786 2.85194062003077 a
    3.48470699044717 3.03599187091698 a
    3.2615625757792 4.40918752625346 a
    3.31908931625676 5.95082391506104 a
    3.40772777457981 1.35402447498146 a
    5.63590334857413 3.23046304809946 b
    3.46418780499208 5.2532962753061 a
    4.81804015863207 3.24356183900056 a
    3.32574801852368 5.34997548719981 a
    2.98254664216517 5.16661394243277 a
    4.57311496229195 4.45931319631445 b
    2.95144223357696 4.76582546007239 a
    2.64874055869206 3.33711558353641 a
    2.86394877458514 4.69859130351621 a
    3.05000367541074 5.73240861105973 a
    3.82181285583226 3.74547112789699 b
    4.4239026177482 2.12757243927978 b
    2.73327988891727 3.04713402219221 a
    3.66697628789954 2.6651037751997 a
    2.68636437091379 3.74003269642794 a
    3.11055071205753 4.27343615977398 a
    3.23061499554796 3.23930038112248 a
    3.03895675529012 3.43560203374447 a
    3.63877987049824 0.402564002310837 a
    2.04678419358542 4.52234144069177 a
    };
    % Begin HyperboxNN
    \addplot[draw=none, surf, mesh/rows=2, patch type=rectangle, fill=red, fill opacity=0.3]
    coordinates {
    (0.0,4.9) (3.65,4.9)
    (0.0,5.1) (3.65,5.1)
    };
    \addplot[surf,mesh/rows=2,patch type=rectangle, fill=red, fill opacity=0.3]
    coordinates {
    (3.65,3.35) (8.0,3.35)
    (3.65,8.0)  (8.0,8.0)
    };
    \addplot[surf,mesh/rows=2,patch type=rectangle, fill=red, fill opacity=0.3]
    coordinates {
    (4.2,0) (8.0,0)
    (4.2,3.2) (8.0,3.2)
    };
    % End HyperboxNN
\end{groupplot}
\end{tikzpicture}
    

==> figures/mainfigure.tex <==
%---
% Define new styles and constants
%---
\tikzstyle{shadednode} = [
    draw,     
    shape=circle,
    densely dashed,
]

\tikzstyle{blacknode} = [
    draw,     
    shape=circle,
    color=black,
    solid, 
]

\tikzstyle{rednode} = [
    draw,     
    shape=circle, 
    color=red,
    solid,
]

\tikzstyle{featuremap} = [
    draw,   
    shape=rectangle,
    fill=gray!10,
    solid,
    align=center,
    minimum height=1.2cm,
    minimum width=2cm,
]

\tikzstyle{index} = [
    draw,
    isosceles triangle,
    isosceles triangle apex angle=60,
    rotate=90,
    fill=white,
    minimum size=1cm,
]

\tikzstyle{indexeddataset} = [
    draw, 
    rectangle, 
    dashed, 
    color=gray, 
    minimum width=9cm, 
    minimum height=1.4cm, 
]

\tikzstyle{query} = [   
    draw, 
    rectangle, 
    dashed, 
    color=gray, 
    minimum width=7cm, 
    minimum height=3cm, 
]

\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{box} = [draw, rectangle, fill=red]
\tikzstyle{customlabel} = [color=black]

\tikzstyle{rare} = [rectangle,
    draw, 
    color=red, 
    minimum width=0.6cm, 
    minimum height=0.6cm,
]

\tikzstyle{nonrare} = [rectangle,
    draw, 
    color=black, 
    minimum width=0.6cm, 
    minimum height=0.6cm,
]
%---

\begin{tikzpicture}[level distance=1.5em,
	level 1/.style={sibling distance=4em},
	level 2/.style={sibling distance=2em},
    node distance=2.2cm and 4cm,
    font=\small]

    \node[query, minimum width=2cm] (nextquery) {};
    \node[query, right=1cm of nextquery] (currentquery) {};
    
	\node[shadednode, below right=0.5cm and -1cm of nextquery] (tree1) {}
	child { node[blacknode] {} edge from parent [dashed]
		child { node[rednode] {}  edge from parent [solid] }
		child { node[blacknode] {} edge from parent [solid]
			child { node[blacknode] {} }
			child { node[rednode] {} }
		}
	}
    child { node[shadednode] {} edge from parent [dashed]
		child { node[shadednode] {} }
		child { node[shadednode] {} }
	};

    \node[shadednode] (tree2) [right=of tree1] {} 
	child { node[shadednode] {} edge from parent [dashed]
		child { node[blacknode] {} edge from parent [solid]
            child { node[rednode] {} }
			child { node[blacknode] {} }
        }
		child { node[shadednode] {} edge from parent [dashed]}
	}
	child { node[blacknode] {} edge from parent [dashed]
		child { node[blacknode] {} edge from parent [solid]}
		child { node[blacknode] {} edge from parent [solid]
			child { node[rednode] {} }
			child { node[blacknode] {} }
		}
	};
    
    \node[shadednode] (tree3) [right=of tree2] {} 
	child { node[blacknode] {} edge from parent [dashed]
		child { node[rednode] {} edge from parent [solid]}
		child { node[blacknode] {} edge from parent [solid]}
	}
	child { node[shadednode] {} edge from parent [dashed]
		child { node[shadednode] {} }
		child { node[blacknode] {} 
            child { node[rednode] {} edge from parent [solid]}
			child { node[blacknode] {} edge from parent [solid]}
		}
	};

    \node[featuremap, below=of tree1] (featuremap1) {};
    \node[featuremap, right=0.7cm of featuremap1] (featuremap2) {};
    \node[featuremap, right=0.7cm of featuremap2] (featuremap21) {};
    \node[featuremap, right=0.7cm of featuremap21] (featuremap3) {};

    \node[index, below right= 1.5cm and -1.3cm of featuremap1] (idx1) {};
    \node[index, below right= 1.5cm and -1.3cm of featuremap2] (idx2) {};
    \node[index, below right= 1.5cm and -1.3cm of featuremap21] (idx21){};  
    \node[index, below right= 1.5cm and -1.3cm of featuremap3] (idx3) {};

    \node[indexeddataset, below right=1.2cm and -1cm of idx1] (idxdataset) {};

    \node[rare, below left=0.9cm and 0cm of idx1] (rare0) {};
    \node[nonrare, right=0.1cm of rare0] (nonrare0) {};
    \node[nonrare, right=0.1cm of nonrare0] (nonrare1){};
    \node[nonrare, right=0.1cm of nonrare1] (nonrare2){};
    \node[nonrare, right=0.1cm of nonrare2] (nonrare3){};
    \node[rare, right=0.1cm of nonrare3] (rare1){};
    \node[nonrare, right=0.1cm of rare1] (nonrare4){};
    \node[rare, right=0.1cm of nonrare4] (rare2){};
    \node[rare, right=0.1cm of rare2] (rare3){};
    \node[nonrare, right=0.1cm of rare3] (nonrare5){};
    

    % Boxes

    % Labels
    \node[customlabel, below=-0.5cm of nextquery] {next query};
    \node[customlabel, below=-0.5cm of currentquery] {current query};
    \node[customlabel, below left=0cm and -0.6cm of featuremap1] {$d_1$};
    \node[customlabel, left=0cm of featuremap1] {$d_7$};
    \node[customlabel, below left=0cm and -0.6cm of featuremap2] {$d_{10}$};
    \node[customlabel, left=0cm of featuremap2] {$d_{23}$};
    \node[customlabel, below left=0cm and -0.6cm of featuremap21] {$d_{6}$};
    \node[customlabel, left=0cm of featuremap21] {$d_{18}$};
    \node[customlabel, below left=0cm and -0.6cm of featuremap3] {$d_{1}$};
    \node[customlabel, left=0cm of featuremap3] {$d_{42}$};
    \node[customlabel, below=-0.5cm of idxdataset] {indexed dataset};
    \node[customlabel, below left=-1.3cm and 0.7cm of idx1, rotate=60] {idx$_{d_{7}d_{1}}$};

    % Dots
    \node[color=black] [below right=0.5cm and 1.5cm of tree1]{\Huge \ldots};
    \node[color=black] (dotslevel1) [below right=0.5cm and 1.5cm of tree2]{\Huge \ldots};
    \node[color=black] [right=0.1cm of featuremap3]{\Huge \ldots};
    \node[color=black] [right=0.1cm of nonrare5]{\Huge \ldots};
    

    % Arrows
    \draw[arrow] (featuremap1) -- (idx1);
    \draw[arrow] (featuremap2) -- (idx2);
    \draw[arrow] (featuremap21) -- (idx21);
    \draw[arrow] (featuremap3) -- (idx3);
    \draw[arrow] (idx1.west) -- (rare0.north);
    \draw[arrow] (idx1.south west) -- (nonrare0.north);
    \draw[arrow] (idx2) -- (nonrare1.north);
    \draw[arrow] (idx2.west) -- (nonrare2.north);
    \draw[arrow] (idx2.south west) -- (nonrare3.north);
    \draw[arrow] (idx2.south west) -- (rare1.north);
    \draw[arrow] (idx21) -- (nonrare4.north); 
    \draw[arrow] (idx21.west) -- (rare2.north);
    \draw[arrow] (idx3.west) -- (rare3.north);
    \draw[arrow] (idx3.south west) -- (nonrare5.north);
    

\end{tikzpicture}

==> text/99_framework.tex <==
%\section{Framework and Background}
%\label{sec:framework_background}
\emph{Problem formulation}: We consider search tasks as user queries given positive and negative examples that can be formulated as (imbalanced) binary classification tasks---one per user query---of the form $\trainset=\{(\vec{x}_1,y_1), \ldots, (\vec{x}_\tsize, y_\tsize)\} \subset \Reals^\tdim \times \Yspace$ with $\Yspace=\{0,1\}$, where a $(\vec{x}_i,y_i)$ with $y_i=1$ corresponds to a desired positive example and $y_i=0$ to a negative example in the training set $\trainset$, see ``user query 1'' and ``user query 2'' on the right side of Figure~\ref{fig:motivation}. Here, $\tdim$~corresponds to the number of features that are extracted per instance. The goal of our search-by-classification approach is to identify all positive instances in a large data catalog.

To make use of multidimensional indexes for fast data retrieval, the classifier to be constructed must attain to the following requirements: be efficient to learn, represent internal decisions as range predicates. These requirements are naturally fulfilled by decision trees and random forests, while exclude deep neural networks, support vector machines, and gradient-boosting algorithms.%\footnote{Adapting deep neural networks to be efficiently supported by index structures is subject to future research, which is out of the scope of our paper.} 

%Decision trees and random forests belong to state-of-the-art classifiers once the features are set (see [15]). Leveraging deep learning approaches such as CNNs or end-to-end trainable object detection frameworks (e.g., YOLO) will generally yield better results, while requiring scanning all the data, which can easily take hours or days, even given powerful (GPU) servers. How to adapt deep neural networks to be efficiently supported by index structures is subject to future research, which is out of the scope of our paper. We will further clarify this in the revised manuscript. 

%\subsection{Search-By-Classification Framework}
Traditional search-by-classification approaches resort to classification models that are built for each new user query. To identify the corresponding positive objects, such models are then typically applied to the entire catalog by scanning all the data.
%Such models are usually applied to the entire data catalog to classify all these instances into rare and non-rare. Thus, typically, a new classification model is built per user query and subsequently applied to the entire catalog by scanning all the data.
%In particular, we consider search tasks defined via an imbalanced classification data set that contains a few rare target and many non-rare instances. 
%The goal is to return all instances in a large collection of data that would be classified as rare by an application of an ML model. 
Our novel search-by-classification framework allows returning these instances \emph{without} scanning the data catalog for each new user query by exploiting index structures pre-built for all instances in the data catalog. %Note that these index structures do \emph{not} depend on the particular user query, \ie, our system can quickly provide the answer for each new task (see Figure~\ref{fig:main_idea}).
%For the sake of exposition, we provide the main algorithmic components of the framework next; the details are provided in Section~\ref{sec:approach}. 
The overall system can be divided into an offline preprocessing and a query processing phase, see Figure~\ref{fig:framework}. 

\begin{figure}
	\centering
	\input{figures/pipeline}
	\caption{Fast search-by-classification via an index-aware classifier and multidimensional index structures pre-built of the data catalog. The index-aware classifier allows implementing the application/inference phase via range queries, which are efficiently supported by the index structures. The target objects can, hence, be obtained via fast spatial lookups instead of a time-consuming scan of all the data.
	%via collaborative design of machine learning models and multi-dimensional index structures. of ML models and indexes: indexes are built to enable accurate search-by-classification, while ML models are designed to efficiently leverage indexes during inference for fast result retrieval.
	}
	\label{fig:framework}
\end{figure}

\subsubsection{Offline Preprocessing}
%\textbf{Feature Extractor}. 
The offline preprocessing phase is only conducted once for the entire data catalog to pre-build the index structures. In a first step, the data are processed via a feature extractor that outputs a $\tdim$-dimensional feature vector per instance in the data catalog (\eg, in the case of image data, these features could be based on information on color, shape, edges, and orientation, see again Figure~\ref{fig:motivation}). 
The extracted features should capture general characteristics of the data and are not tailored to any specific query.\footnote{For image data, such features can be extracted in an automatic manner via, e.g., pre-trained or unsupervised deep neural networks, see Section~\ref{sec:experiments}.}
%In an offline phase, we transform raw data in the original database into features that help the downstream classifier to accurately distinguish data objects. 
Afterwards, a pre-defined number $\tsizesubsets$ of index structures are built via an index builder. Here, one indexing structure is generated for a corresponding random feature subset containing a few features (\eg, given $\tdim=100$ features, $\text{idx}_1$ could be an index for the feature subset $\{17,51,60,80\}$, $\text{idx}_2$ an index for $\{11,45,49,99\}$, and so on).
%Here, a moderate number of features are used per index (\eg, three or four).
%\textbf{Index Builder}. We generate a number of indexes for random subsets of features extracted in the previous step.
As described below, the index structures are taken into account during the construction of the classification models in the query processing phase. %\footnote{\todot{Fabian: Here, we already provide an implementation detail. Maybe move to experiments section?} The main challenge in this step lies on providing a sufficient number of feature subsets to the downstream classifier in order to enable high accuracy in the query results, while keeping a moderate number of generated indexes to reduce the space consumption overhead. This overhead is acceptable since storage costs are often cheaper than processing costs, especially in cloud-based systems~\cite{Bello2021cloud}, and can be further alleviated via compressed indexes~\cite{Arroyuelo2022compridx}.} 


% in order to achieve high accuracy in the query results, we need to provide the downstream classifier with a sufficient number of feature subsets. In contrast, to achieve high efficiency, a moderate number of features are used in each index (e.g., three or four). On the other hand, since building indexes creates an overhead in space consumption, we need to maintain the number of indexes\todot{Discuss why the overhead is acceptable, and possible approach to further reduce the storage overhead.}  
% \newtext{
% \textbf{Query Processing}. In the online phase, user queries composed by a training set of positive- and negative-labeled data is transformed using the same feature extractor used in the offline phase.
% }

\subsubsection{Query Processing} 
In this phase, each user query is defined via a small set of positive and negative training examples (\eg, image patches with wind turbines and other objects, respectively). In the first step of the query processing phase, the feature extractor used in the offline preprocessing phase is used to extract a feature vector for each element of the training set.
%The main task our framework has to perform is to learn a classifier that properly distinguishes rare from non-rare training examples included in user queries. 
%\textbf{Index-Aware Classifier}. 
Next, a novel ``index-aware'' classifier is built for the given training data. In a nutshell, information about the indexes built in the offline preprocessing phase are considered during the construction (dashed lines in Figure~\ref{fig:framework}) such that the catalog instances being classified as ``positive'' can be efficiently retrieved via orthogonal range queries, supported by a corresponding index structure (solid lines).
%using the feature subsets used in the offline phase.
%More precisely, hyperboxes that cover data objects assigned with the ``rare'' class label.
%These hyperboxes are transformed into range queries that leverage the pre-build indexes for fast data retrieval (see Section~\ref{sec:rare_leaves_range_queries}).
%to efficiently retrieve the target data. Second, it should be efficient to train, since for each user query a new classifier must be built. Third, the classifier should allow for directly expressing its decisions in SQL. Decision trees, random forests, and other forms of rule-based classifiers are natural candidates in this context~\cite{tran2009qbo}. 
%Here, we introduce an alternative bottom-up construction scheme for decision trees and random forests, which yields, per user query, a corresponding set of range queries. 
%From the learned classifier, we extract a set of hyperboxes that cover data objects assigned with the ``rare'' class label.
%These hyperboxes are transformed into range queries that leverage the pre-build indexes for fast data retrieval (see Section~\ref{sec:rare_leaves_range_queries}).
%Finally, the range queries are efficiently executed by means of the corresponding index structures (solid lines). 
The overall pipeline can, per user query, return the desired classification results in a fraction of the time that would be needed by a full scan of the data catalog.
The corresponding details will be provided in Section~\ref{sec:approach}.

